Observability and Chaos Engineering on System Calls for Containerized Applications in Docker

In this paper, we present a novel fault injection system called ChaosOrca for system calls in containerized applications. ChaosOrca aims at evaluating a given application's self-protection capability with respect to system call errors. The unique feature of ChaosOrca is that it conducts experiments under production-like workload without instrumenting the application. We exhaustively analyze all kinds of system calls and utilize different levels of monitoring techniques to reason about the behaviour under perturbation. We evaluate ChaosOrca on three real-world applications: a file transfer client, a reverse proxy server and a micro-service oriented web application. Our results show that it is promising to detect weaknesses of resilience mechanisms related to system calls issues.

==> tables/summary-bookinfo.tex <==
\begin{table*}[pos=t]
\centering
\caption{A Sample of Chaos Experiments on Bookinfo (In The First Column, D = delay, E = error)}\label{tab:summary-bookinfo}
\scriptsize
\begin{tabular*}{\textwidth}{lllp{5.5cm}}
\toprule
Perturbation Model& Trend of HTTP Requests& Trend of System Calls& Other findings\\
\midrule
Open + D&Fewer 200&Normal, increase for 5s delay&Increased CPU usage\\
Open + E&Fewer 200&Normal or fewer&Smaller Network IO. Increased CPU.\\
Open + E + D&Fewer to very few 200.&Normal/increase, spike after&Small Network IO. Increased CPU.\\
Write + D&Very few to no 200&Normal and spike after&Small network IO. Normal+spike CPU.\\
Write + E&Fewer 200, no 302&Normal/increase&Smaller network IO. Increased CPU.\\
Write + E + D&None, up after&Normal and spike after&Smaller network IO, normal CPU, both spike after\\
Read + D&Fewer to none. Up after.&Increase. +spike for 5s delay&Smaller Network IO, increased CPU. +spike for 5s delay\\
Read + E&No request&Normal/fewer. EINTR increase spike&normal. EINTR Network IO small. CPU increase.\\
Read + E + D&None, up after&Normal and spike after&Both Network IO and CPU small+spike.\\
Poll + D&Fewer to few 200. &Increase. +spike for 5s delay&Smaller Network IO, increased CPU. +spike for 5s delay\\
Poll + E&Fewer 200. None for EINTR&Fewer/normal. Very few+spike for EINTR&Smaller Network IO, increased CPU. big CPU+spike for EINTR\\
Poll + E + D&Few 200, up after&Increase and spike after&Small Network IO, increased CPU\\
Select + D&Few to none 200, up after&Normal/tiny and spike after&Tiny+spike Network IO, small+spike CPU.\\
Select + E&crash. EINTR none, up after&EINTR increase+spike&Tiny+spike Network IO, huge CPU.\\
Select + E + D&crash &EINTR crash after perturb.&\\
\bottomrule
\end{tabular*}
\end{table*}

==> tables/summary-nginx.tex <==
\begin{table*}[pos=t]
\centering
\caption{A Sample of Chaos Experiments on Nginx (In The First Column, D = delay, E = error)}\label{tab:summary-nginx}
\scriptsize
\begin{tabular*}{\textwidth}{lp{4.5cm}p{4.5cm}p{4.5cm}}
\toprule
Perturbation Model& Trend of HTTP Requests& Trend of System Calls& Other findings\\
\midrule
Open + D& Very few successful requests& Fewer and spike after& Both CPU and Network IO is tiny during and spike after\\
Open + E& Error code differ on injected Error& Fewer& \\
Open + E + D& Fewer requests, error code differ on injected error& A lot less and spike after& Both CPU and Network IO is tiny during and spike after\\
Write + D& No successful requests& Fewer and spike after& Both CPU and Network IO is tiny during and spike after\\
Write + E& & & Slight increase in CPU usage\\
Write + E + D& Fewer successful requests, 5s delay essentially none& Fewer and spike after& Both CPU and Network IO is tiny during and spike after\\
Writev + D& Few successful requests& Fewer and spike after& Both CPU and Network IO is tiny during and spike after\\
Writev + E& No successful requests& Normal except for EINTR with fewer and spike after& Low Network IO\\
Writev + E + D& No successful requests& Fewer and spike after& Both CPU and Network IO is tiny during and spike after\\
Sendfile + D& No successful requests& Fewer and spike after& Both CPU and Network IO is tiny during and spike after\\
Sendfile + E& No successful requests& Normal except for EINTR with fewer and spike after& As above except for EINTR with high cpu usage\\
Sendfile + E + D& No successful requests& Fewer and spike after& Both CPU and Network IO is tiny during and spike after\\
\bottomrule
\end{tabular*}
\end{table*}

==> tables/summary-ttorrent.tex <==
\begin{table*}[pos=t]
\centering
\caption{A Sample of Chaos Experiments on TTorrent (In The First Column, D = delay, E = error)}\label{tab:summary-ttorrent}
\scriptsize
\begin{tabular*}{\textwidth}{lll}
\toprule
Perturbation Model& Trend of System Calls& Other findings\\
\midrule
Open + D& Increase after& Network IO dips down during\\
Open + E& Mostly normal& Network IO normal\\
Open + E + D& In general increase& Network IO dips with high delay. CPU increase\\
Write + D& Fewer syscalls during& Network IO dips during\\
Write + E& Fewer syscalls during, few to none after. EINTR only dips& Network IO stops. EINTR only dips.\\
Write + E + D& Very few syscalls, few to none after. EINTR small dip& Network IO stops. EINTR dips then to small.\\
Read + D& Big dip during& Network IO big dip during, \\
Read + E& Very few syscalls, few to none after. EINTR big dip& Network IO stops. EINTR dips then to small\\
Read + E + D& Very few syscalls, few to none after.& Network IO stops. Tiny CPU.\\
\bottomrule
\end{tabular*}
\end{table*}
